Diagnosing and Stabilizing RLVR Training through Entropy Dynamics

Reinforcement Learning with Verifiable Rewards (RLVR) is a central component of modern LLM post-training, yet the training is prone to instability and collapse. Prior work has largely studied this instability through the lens of off-policiness, but the resulting mitigation strategies do not consistently stabilize training across settings. Rather than attributing instability to a particular training-inference mismatch, we take a complementary approach that characterizes and directly controls a common signature of collapse. Across models and datasets, we find that RLVR collapse is consistently associated with a sharp increase in entropy. We use a first-order estimate of entropy change from the policy gradient and show that, it follows the same qualitative trend as the observed entropy prior to collapse. Directly controlling updates according to this quantity produces consistent improvements in training stability across models and datasets. We further find that the effectiveness of existing stabilization strategies is closely associated with their ability to control this entropy-gradient signal, providing a common explanation for when these interventions succeed or fail. Together, these results provide an entropy-based perspective on RLVR instability and suggest that controlling entropy growth is a key ingredient for stable training.

==> plots/correlation/correlation.tex <==
% Directly include this file in the paper with:
% \input{plots/correlation/correlation.tex}
%
% Required in the paper preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \pgfplotsset{compat=1.18}
%
% Data source and extraction details are in extract_correlation_data.py.

\begin{figure*}[t]
\centering

\definecolor{Blue}{HTML}{0072B2}
\definecolor{Orange}{HTML}{E69F00}
\definecolor{Red}{HTML}{D55E00}
\definecolor{Sky}{HTML}{56B4E9}
\definecolor{Gray}{HTML}{6B7280}

% Override this before \input when the paper is compiled from another root.
\providecommand{\CorrelationDataDir}{plots/correlation/data}

\pgfmathsetlengthmacro{\CorrelationPanelWidth}{0.36*\hsize}
\pgfmathsetlengthmacro{\CorrelationPanelHeight}{0.30*\hsize}
% Change only this definition to rename the metric everywhere in this figure.
\def\FirstOrderEntropyChangeLabel{$\Delta H_{\mathrm{sum}}$}
\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=3 by 1,
      horizontal sep=0.75cm,
    },
    width=\CorrelationPanelWidth,
    height=\CorrelationPanelHeight,
    xmin=0,
    xmax=200,
    xtick={0,50,100,150,200},
    xlabel={Training step},
    grid=major,
    grid style={Gray!18},
    axis line style={Gray!70},
    tick style={Gray!70},
    tick label style={font=\small},
    label style={font=\small},
    title style={font=\small, yshift=-0.5ex, align=center},
  ]
    \nextgroupplot[
      title={\textbf{(a)} \FirstOrderEntropyChangeLabel},
      ymin=-0.013,
      ymax=0.006,
      ytick={-0.012,-0.008,-0.004,0,0.004},
      scaled y ticks=false,
      yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},
    ]
      \addplot+[Blue, very thick, no marks]
        table[x=step, y=entropy_change_sum]
        {\CorrelationDataDir/correlation.dat};

    \nextgroupplot[
      title={\textbf{(b)} Mean policy entropy $H_t$},
      ymin=0,
      ymax=12,
      ytick={0,2,4,6,8,10,12},
    ]
      \addplot+[Blue, very thick, no marks]
        table[x=step, y=mean_policy_entropy]
        {\CorrelationDataDir/correlation.dat};

    \nextgroupplot[
      title={\textbf{(c)} Train reward},
      ymin=0,
      ymax=0.52,
      ytick={0,0.1,0.2,0.3,0.4,0.5},
    ]
      \addplot+[Blue, very thick, no marks]
        table[x=step, y=reward]
        {\CorrelationDataDir/correlation.dat};
  \end{groupplot}
\end{tikzpicture}

\caption{%
  Training dynamics of the OTT-Qwen DR-DAPO baseline
  (\texttt{ott-qwen-drdapo-bf16}). From left to right, the panels report
  \FirstOrderEntropyChangeLabel, mean policy entropy $H_t$, and train reward.
  Curves show the raw logged values over 200 training steps without smoothing.%
}
\label{fig:correlation}
\end{figure*}


==> plots/eighty_twenty_rule/eighty_twenty_rule.tex <==
% Directly include this file in the paper with:
% \input{plots/eighty_twenty_rule/eighty_twenty_rule_plot.tex}
%
% Required in the paper preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \pgfplotsset{compat=1.18}
%
% Data source and extraction details are in extract_eighty_twenty_data.py.

\begin{figure*}[t]
\centering

\definecolor{Blue}{HTML}{0072B2}
\definecolor{Orange}{HTML}{E69F00}
\definecolor{Red}{HTML}{D55E00}
\definecolor{Sky}{HTML}{56B4E9}
\definecolor{Gray}{HTML}{6B7280}

% Override this before \input when the paper is compiled from another root.
\providecommand{\EightyTwentyDataDir}{plots/eighty_twenty_rule/data}

% Change only this definition to rename the metric everywhere in this figure.
\def\FirstOrderEntropyChangeLabel{First-order entropy change sum}
\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=2 by 1,
      horizontal sep=1.80cm,
    },
    width=0.42\textwidth,
    height=0.31\textwidth,
    xmin=0,
    xmax=200,
    xtick={0,50,100,150,200},
    xlabel={Training step},
    grid=major,
    grid style={Gray!18},
    axis line style={Gray!70},
    tick style={Gray!70},
    tick label style={font=\small},
    label style={font=\small},
    legend style={
      draw=none,
      font=\small,
      legend columns=-1,
      /tikz/every even column/.append style={column sep=0.8em},
    },
  ]
    \nextgroupplot[
      ylabel={\FirstOrderEntropyChangeLabel},
      ymin=-0.013,
      ymax=0.006,
      ytick={-0.012,-0.008,-0.004,0,0.004},
      legend to name=eightytwentylegend,
    ]
      \addplot+[
        color=Blue, very thick, solid,
        mark=*, mark size=1.8pt, mark repeat=20,
        mark options={draw=Blue, fill=Blue}
      ]
        table[x=step, y=first_order_entropy_change_sum]
        {\EightyTwentyDataDir/baseline.dat};
      \addlegendentry{Baseline}

      \addplot+[
        color=Orange, very thick, dashed,
        mark=square*, mark size=1.8pt, mark repeat=20,
        mark options={draw=Orange, fill=Orange}
      ]
        table[x=step, y=first_order_entropy_change_sum]
        {\EightyTwentyDataDir/eighty_twenty.dat};
      \addlegendentry{80/20 rule}

    \nextgroupplot[
      ylabel={Exact-match reward},
      ymin=0,
      ymax=0.32,
      ytick={0,0.05,0.10,0.15,0.20,0.25,0.30},
      yticklabel style={
          /pgf/number format/fixed,
          /pgf/number format/precision=2,
          /pgf/number format/fixed zerofill,
        }
    ]
      \addplot+[
        color=Blue, very thick, solid,
        mark=*, mark size=1.8pt, mark repeat=20,
        mark options={draw=Blue, fill=Blue}
      ]
        table[x=step, y=em_reward]
        {\EightyTwentyDataDir/baseline.dat};

      \addplot+[
        color=Orange, very thick, dashed,
        mark=square*, mark size=1.8pt, mark repeat=20,
        mark options={draw=Orange, fill=Orange}
      ]
        table[x=step, y=em_reward]
        {\EightyTwentyDataDir/eighty_twenty.dat};
  \end{groupplot}

  \path (group c1r1.north west) --
    node[anchor=south, yshift=2mm]
      {\pgfplotslegendfromname{eightytwentylegend}}
    (group c2r1.north east);
\end{tikzpicture}

\caption{%
  Effect of the 80/20 entropy masking rule on training dynamics. The baseline
  is shown for 200 training steps, while the 80/20 run contains 110 logged
  steps. The left panel reports
  \FirstOrderEntropyChangeLabel, and the right panel reports exact-match
  reward. Curves show the raw logged values without smoothing.%
}
\label{fig:eighty-twenty-training-dynamics}
\end{figure*}


==> plots/gac_experiment/gac_experiment_plot.tex <==
% Directly include this file in the paper with:
% \input{plots/gac_experiment/gac_experiment_plot.tex}
%
% Required in the paper preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \pgfplotsset{compat=1.18}
%
% Data source and extraction details are in extract_gac_data.py.

\begin{figure*}[t]
\centering

\definecolor{Blue}{HTML}{0072B2}
\definecolor{Orange}{HTML}{E69F00}
\definecolor{Red}{HTML}{D55E00}
\definecolor{Sky}{HTML}{56B4E9}
\definecolor{Gray}{HTML}{6B7280}

% Override this before \input when the paper is compiled from another root.
\providecommand{\GACDataDir}{plots/gac_experiment/data}

% Change only this definition to rename the metric everywhere in this figure.
\def\FirstOrderEntropyChangeLabel{First-order entropy change sum}
\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=2 by 1,
      horizontal sep=1.25cm,
    },
    width=0.43\textwidth,
    height=0.31\textwidth,
    xmin=0,
    xmax=500,
    xtick={0,100,200,300,400,500},
    xlabel={Training step},
    grid=major,
    grid style={Gray!18},
    axis line style={Gray!70},
    tick style={Gray!70},
    tick label style={font=\small},
    label style={font=\small},
    legend style={
      draw=none,
      font=\small,
      legend columns=-1,
      /tikz/every even column/.append style={column sep=0.8em},
    },
  ]
    \nextgroupplot[
      ylabel={\FirstOrderEntropyChangeLabel},
      ymin=0,
      ymax=0.045,
      legend to name=gaclegend,
    ]
      \addplot+[
        color=Blue, very thick, solid,
        mark=*, mark size=1.8pt, mark repeat=25,
        mark options={draw=Blue, fill=Blue}
      ]
        table[x=step, y=first_order_entropy_change_sum]
        {\GACDataDir/s8.dat};
      \addlegendentry{Baseline}

      \addplot+[
        color=Orange, very thick, dashed,
        mark=square*, mark size=1.8pt, mark repeat=25,
        mark options={draw=Orange, fill=Orange}
      ]
        table[x=step, y=first_order_entropy_change_sum]
        {\GACDataDir/s1_on_policy.dat};
      \addlegendentry{On-policy}

    \nextgroupplot[
      ylabel={Train reward},
      ymin=0,
      ymax=1.05,
      ytick={0,0.2,0.4,0.6,0.8,1.0},
    ]
      \addplot+[
        color=Blue, very thick, solid,
        mark=*, mark size=1.8pt, mark repeat=25,
        mark options={draw=Blue, fill=Blue}
      ]
        table[x=step, y=train_reward]
        {\GACDataDir/s8.dat};

      \addplot+[
        color=Orange, very thick, dashed,
        mark=square*, mark size=1.8pt, mark repeat=25,
        mark options={draw=Orange, fill=Orange}
      ]
        table[x=step, y=train_reward]
        {\GACDataDir/s1_on_policy.dat};
  \end{groupplot}

  \path (group c1r1.north west) --
    node[anchor=south, yshift=2mm] {\pgfplotslegendfromname{gaclegend}}
    (group c2r1.north east);
\end{tikzpicture}

\caption{%
  Training dynamics of the 8 step off-policy baseline and zero policy lag GAC experiments. The baseline collapses reports the training curve before collapse near step 100, and the GAC method is shown for 500 training steps. The left panel reports \FirstOrderEntropyChangeLabel, and
  the right panel reports train reward. The GAC run is stable with a lower \FirstOrderEntropyChangeLabel at each training step. Curves show the raw logged values without smoothing.%
}
\label{fig:gac-training-dynamics}
\end{figure*}


==> plots/main_results/main_results.tex <==
% Directly include this file in the paper with:
% \input{plots/main_results/main_results_plot.tex}
%
% Required in the paper preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \pgfplotsset{compat=1.18}
%
% Data source and deterministic extraction details are in
% plots/main_results/extract_main_results_data.py.

\begin{figure*}[t]
\centering

\definecolor{Blue}{HTML}{0072B2}
\definecolor{Orange}{HTML}{E69F00}
\definecolor{Red}{HTML}{D55E00}
\definecolor{Sky}{HTML}{56B4E9}
\definecolor{Gray}{HTML}{6B7280}

% Override this before \input when the paper is compiled from another root.
\providecommand{\MainResultsDataDir}{plots/main_results/data}

% Size the axes themselves relative to the include context's column-sized
% \hsize; the four compact panels and their gaps fit across the figure* width.
% Do not scale the surrounding TikZ picture, since that would scale typography.
\pgfmathsetlengthmacro{\MainResultsPanelWidth}{0.3*\hsize}
\pgfmathsetlengthmacro{\MainResultsPanelHeight}{0.24*\hsize}
% Change only this definition to rename the metric everywhere in this figure.
\def\FirstOrderEntropyChangeLabel{$\widehat{\Delta H}_{\mathrm{sum}}$}
\begin{tikzpicture}
  \begin{groupplot}[
      group style={
      group size=4 by 2,
      horizontal sep=0.75cm,
      vertical sep=1.50cm,
    },
    width=\MainResultsPanelWidth,
    height=\MainResultsPanelHeight,
    xmin=0,
    xmax=500,
    unbounded coords=jump,
    xtick={0,100,200,300,400,500},
    grid=major,
    grid style={Gray!18},
    axis line style={Gray!70},
    tick style={Gray!70},
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small, yshift=-0.5ex},
    scaled y ticks=false,
    yticklabel style={
      font=\scriptsize,
      /pgf/number format/fixed,
      /pgf/number format/precision=3,
      /pgf/number format/skip 0.=false,
    },
    legend style={
      draw=none,
      font=\small,
      legend columns=-1,
      /tikz/every even column/.append style={column sep=1.0em},
    },
  ]
    \nextgroupplot[
      title={\FirstOrderEntropyChangeLabel},
      ymin=-0.02,
      ymax=0.01,
      ytick={-0.02,-0.01,0,0.01},
      legend to name=mainresultslegend,
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=ott_baseline_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addlegendentry{Baseline}
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=ott_pec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addlegendentry{$\widehat{\Delta H} < \tau^{+}$}
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=ott_pec_nec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addlegendentry{$\tau^{-} < \widehat{\Delta H} < \tau^{+}$}

    \nextgroupplot[
      title={Exact-match reward},
      ymin=0,
      ymax=0.65,
      ytick={0,0.2,0.4,0.6},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=ott_baseline_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=ott_pec_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=ott_pec_nec_reward] {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={\FirstOrderEntropyChangeLabel},
      ymin=-0.002,
      ymax=0.0055,
      ytick={-0.002,0,0.002,0.004},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=math_gemma_baseline_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=math_gemma_pec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=math_gemma_pec_nec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={Train reward},
      ymin=0,
      ymax=0.9,
      ytick={0,0.2,0.4,0.6,0.8},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=math_gemma_baseline_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=math_gemma_pec_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=math_gemma_pec_nec_reward] {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={\FirstOrderEntropyChangeLabel},
      xlabel={Training step},
      ymin=-0.005,
      ymax=0.019,
      ytick={-0.005,0,0.005,0.01,0.015},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=numina_qwen_baseline_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=numina_qwen_pec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=numina_qwen_pec_nec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={Train reward},
      xlabel={Training step},
      ymin=0,
      ymax=0.72,
      ytick={0,0.2,0.4,0.6},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=numina_qwen_baseline_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=numina_qwen_pec_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=numina_qwen_pec_nec_reward] {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={\FirstOrderEntropyChangeLabel},
      xlabel={Training step},
      ymin=-0.0015,
      ymax=0.011,
      ytick={-0.001,0,0.004,0.008},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=numina_gemma_baseline_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=numina_gemma_pec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=numina_gemma_pec_nec_first_order_entropy_change_sum]
        {\MainResultsDataDir/main_results.dat};

    \nextgroupplot[
      title={Train reward},
      xlabel={Training step},
      ymin=0,
      ymax=0.65,
      ytick={0,0.2,0.4,0.6},
    ]
      \addplot+[Blue, very thick, solid, no marks]
        table[x=step, y=numina_gemma_baseline_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Orange, very thick, dashed, no marks]
        table[x=step, y=numina_gemma_pec_reward] {\MainResultsDataDir/main_results.dat};
      \addplot+[Red, very thick, dash dot, no marks]
        table[x=step, y=numina_gemma_pec_nec_reward] {\MainResultsDataDir/main_results.dat};
  \end{groupplot}

  \path (group c1r1.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(a) OTT-QA--Qwen}
    (group c2r1.north east);
  \path (group c3r1.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(b) MATH--Gemma}
    (group c4r1.north east);
  \path (group c1r2.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(c) Numina--Qwen}
    (group c2r2.north east);
  \path (group c3r2.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(d) Numina--Gemma}
    (group c4r2.north east);
  \path (group c1r2.south west) --
    node[anchor=north, yshift=-8mm] {\pgfplotslegendfromname{mainresultslegend}}
    (group c4r2.south east);
\end{tikzpicture}

\caption{%
  Main training results for the baseline, entropy-increasing updates filter $\widehat{\Delta H} < \tau^{+}$, and
  combined entropy-increasing/decreasing updates filter change $\tau^{-} < \widehat{\Delta H} < \tau^{+}$.
  Each two-panel block reports the two training metrics over at most 500
  training steps. We used $\tau^{+}=0.2$ for OTT-QA/Qwen3-4B experiments, $\tau^{+}=0.1$ for other three dataset-model combinations, and $\tau^{-}=-0.1$ for all experiments.
}
\label{fig:main-training-results}
\end{figure*}


==> plots/on-policy-entropy-stability/plot.tex <==
% Directly include this file in the paper with:
% \input{plots/on-policy-entropy-stability/plot.tex}
%
% Required in the paper preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \pgfplotsset{compat=1.18}
%
% Run IDs:
% GAC: badwlmu2 + v84s7bnf (on-policy continuation), q91aoq2e (s=8)
% Numina--Qwen: e6otnobo (on-policy), 319gs1q5 (off-policy, s=4)

\begin{figure*}[t]
\centering

\definecolor{StabilityBlue}{HTML}{0072B2}
\definecolor{StabilityOrange}{HTML}{E69F00}
\definecolor{StabilityGray}{HTML}{6B7280}

\providecommand{\OnPolicyStabilityDataDir}{plots/on-policy-entropy-stability/data}

\pgfmathsetlengthmacro{\OnPolicyStabilityPanelWidth}{0.35\textwidth}
\pgfmathsetlengthmacro{\OnPolicyStabilityPanelHeight}{0.25\textwidth}

\begin{tikzpicture}
  \begin{groupplot}[
    group style={
      group size=3 by 2,
      horizontal sep=0.9cm,
      vertical sep=1.55cm,
    },
    width=\OnPolicyStabilityPanelWidth,
    height=\OnPolicyStabilityPanelHeight,
    xmin=0,
    xmax=200,
    xtick={0,50,100,150,200},
    xlabel={Gradient steps},
    unbounded coords=jump,
    grid=major,
    grid style={StabilityGray!18},
    axis line style={StabilityGray!70},
    tick style={StabilityGray!70},
    tick label style={font=\scriptsize},
    label style={font=\small},
    title style={font=\small, yshift=-0.5ex},
    scaled y ticks=false,
    yticklabel style={
      font=\scriptsize,
      /pgf/number format/fixed,
      /pgf/number format/precision=3,
      /pgf/number format/skip 0.=false,
    },
    legend style={
      draw=none,
      font=\scriptsize,
      cells={anchor=west},
    },
  ]
    % GAC row
    \nextgroupplot[
      title={Reward},
      xmax=500,
      xtick={0,100,200,300,400,500},
      ymin=0,
      ymax=1.05,
      ytick={0,0.25,0.5,0.75,1},
      legend pos=south east,
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=reward, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-on-policy.csv};
      \addlegendentry{On-policy ($s=1$)}
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=reward, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-s8.csv};
      \addlegendentry{GAC ($s=8$)}

    \nextgroupplot[
      title={Entropy},
      xmax=500,
      xtick={0,100,200,300,400,500},
      ymin=0.1,
      ymax=0.28,
      ytick={0.1,0.14,0.18,0.22,0.26},
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=entropy, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-on-policy.csv};
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=entropy, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-s8.csv};

    \nextgroupplot[
      title={Accumulated first-order entropy change},
      xmax=500,
      xtick={0,100,200,300,400,500},
      ymin=0,
      ymax=2.6,
      ytick={0,0.5,1,1.5,2,2.5},
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=cumulative_first_order_entropy_change, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-on-policy.csv};
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=cumulative_first_order_entropy_change, col sep=comma]
        {\OnPolicyStabilityDataDir/gac-s8.csv};

    % Numina--Qwen row
    \nextgroupplot[
      title={Reward},
      ymin=0,
      ymax=0.75,
      ytick={0,0.2,0.4,0.6},
      legend pos=north west,
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=reward, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-on-policy.csv};
      \addlegendentry{On-policy ($s=1$)}
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=reward, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-off-policy.csv};
      \addlegendentry{Off-policy ($s=4$)}

    \nextgroupplot[
      title={Entropy},
      ymin=0.25,
      ymax=1.8,
      ytick={0.4,0.8,1.2,1.6},
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=entropy, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-on-policy.csv};
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=entropy, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-off-policy.csv};

    \nextgroupplot[
      title={Accumulated first-order entropy change},
      ymin=-0.003,
      ymax=0.014,
      ytick={0,0.004,0.008,0.012},
    ]
      \addplot[StabilityBlue, very thick, solid, no marks]
        table[x=gradient_step, y=cumulative_first_order_entropy_change, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-on-policy.csv};
      \addplot[StabilityOrange, very thick, dashed, no marks]
        table[x=gradient_step, y=cumulative_first_order_entropy_change, col sep=comma]
        {\OnPolicyStabilityDataDir/numina-qwen-off-policy.csv};
  \end{groupplot}

  \path (group c1r1.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(a) GAC}
    (group c3r1.north east);
  \path (group c1r2.north west) --
    node[anchor=south, yshift=5mm, font=\small\bfseries] {(b) Numina--Qwen}
    (group c3r2.north east);
\end{tikzpicture}

\caption{%
  Reward, policy entropy, and accumulated first-order entropy change for
  on-policy and multi-step policy optimization. The horizontal axis reports
  optimizer gradient steps. Logged steps map one-to-one to gradient steps for
  the on-policy runs and to four gradient steps for both comparison runs. The
  GAC row shows 500 gradient steps, including the continuation of the
  on-policy run, while the Numina--Qwen row shows 200 gradient steps.
}
\label{fig:on-policy-entropy-stability}
\end{figure*}

